Conquering the Extensional Scalability Problem for Value-Flow Analysis Frameworks

With an increasing number of value-flow properties to check, existing static program analysis still tends to have scalability issues when high precision is required. We observe that the key design flaw behind the scalability problem is that the core static analysis engine is oblivious of the mutual synergies among different properties being checked and, thus, inevitably loses many optimization opportunities. Our approach is inter-property-aware and able to capture possible overlaps and inconsistencies among different properties. Thus, before analyzing a program, we can make optimization plans which decide how to reuse the specific analysis results of a property to speed up checking other properties. Such a synergistic interaction among the properties significantly improves the analysis performance. We have evaluated our approach by checking twenty value-flow properties in standard benchmark programs and ten real-world software systems. The results demonstrate that our approach is more than 8x faster than existing ones but consumes only 1/7 memory. Such a substantial improvement in analysis efficiency is not achieved by sacrificing the effectiveness: at the time of writing, 39 bugs found by our approach have been fixed by developers and four of them have been assigned CVE IDs due to their security impact.

==> pre.tex <==
\section{Preliminaries}
\label{sec:preliminaries}


With no loss of generality, we assume the code in each function is in static single assignment (SSA) form, where every variable has only one definition~\cite{cytron1989efficient}.
In a program, as existing work~\cite{li2011boosting,sui2014detecting,shi2018pinpoint},  
we say the value of a variable $a$ flows to a variable $b$ (or $b$ is data-dependent on $a$) if 
$a$ is assigned to $b$ directly (via an assignment, such as \textit{b=a}) or indirectly (via pointer dereferences, such as \textit{*p=a; q=p; b=*q}).
Then, the value-flow graph is defined as below.

\begin{definition}[Value-Flow Graph]
	A value-flow graph is a directed graph $G = (V, E)$, where $V$ and $E$ are defined as following:
	\begin{itemize}
		\item $V$ is a set of vertices, each of which is denoted by $v@s$, meaning the variable $v$ is defined or used in the statement $s$.
		To be clear, we simply write $v$ or $s$ if it does not cause any confusion such as in the case of Figure~\ref{fig:sec2_example}.
		
		\smallskip
		
		\item $E\subseteq V\times V$ is a set of edges, each of which represents a data dependence relation or value flow. 
		$(v_1@s_1, v_2@s_2)\in E$ means that the value of $v_1@s_1$ flows to $v_2@s_2$.
	\end{itemize}
	\label{def:vfg}
\end{definition}

We say $\pi =   (v_0@s_0, v_1@{s_1}, \cdots, v_n@{s_n} )$ is a value-flow path
iff the sequence represents a path on the value-flow graph.
We use $\pi[i]$ to represent $v_i@{l_i}$ on the path if $0\le i\le n$. 
Specifically, we use $\pi[-1]$ to represent the last element of $\pi$.
A value-flow path $\pi_2$ can be concatenated to the other one $\pi_1$, denoted as $\pi_1\pi_2$,
iff $(\pi_1[-1], \pi_2[0]) \in E$.
Given $V_1, V_2\subseteq V$, we use $\Pi(V_1, V_2)$ to represent the set of value-flow paths from a vertex in $V_1$ to a vertex in $V_2$.

%Given $V_1, V_2, V_3, V_4\subseteq V$, we use $\Pi(V_1, V_2)$ to represent the set of value-flow paths from a vertex in $V_1$ to a vertex in $V_2$.
%The concatenation of two value-flow paths then can be extended to two sets:
%$\Pi(V_1, V_2)\Pi(V_3, V_4)=\{\pi_1\pi_2:  \pi_1\in \Pi(V_1, V_2) \land \pi_2\in \Pi(V_3, V_4) \land (\pi_1[-1], \pi_2[0])\in E\}.$



